Intuitive Human-Drone Collaborative Navigation in Unknown Environments through Mixed Reality

Considering the widespread integration of aerial robots in inspection, search and rescue, and monitoring tasks, there is a growing demand to design intuitive human-drone interfaces. These aim to streamline and enhance the user interaction and collaboration process during drone navigation, ultimately expediting mission success and accommodating users' inputs. In this paper, we present a novel human-drone mixed reality interface that aims to (a) increase human-drone spatial awareness by sharing relevant spatial information and representations between the human equipped with a Head Mounted Display (HMD) and the robot and (b) enable safer and intuitive human-drone interactive and collaborative navigation in unknown environments beyond the simple command and control or teleoperation paradigm. We validate our framework through extensive user studies and experiments in a simulated post-disaster scenario, comparing its performance against a traditional First-Person View (FPV) control systems. Furthermore, multiple tests on several users underscore the advantages of the proposed solution, which offers intuitive and natural interaction with the system. This demonstrates the solution's ability to assist humans during a drone navigation mission, ensuring its safe and effective execution.

==> notation.tex <==
%!TEX root = ARTICLE.tex

\DeclareMathOperator{\sgn}{sgn}

% Frame Notation
\newcommand{\camf}{\mathcal{C}}
\newcommand{\robotf}{\mathcal{B}}
\newcommand{\worldf}{\mathcal{I}}
\newcommand{\loadf}{\mathcal{L}}

% Vector
\newcommand{\deltat}{\Delta t}
\newcommand{\veca}{\boldsymbol{a}}
\newcommand{\vecam}{\veca_m}
\newcommand{\vecba}{\mathbf{b}_a}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\vecc}{\mathbf{c}}
\newcommand{\vecd}{\mathbf{d}}
\newcommand{\vece}{\mathbf{e}}
\newcommand{\vecF}{\mathbf{F}}
\newcommand{\vecbyaw}{\vecb^{yaw}}
\newcommand{\vecbSxdes}{\vecb_{1S}^*}
\newcommand{\vecbSydes}{\vecb_{2S}^*}
\newcommand{\vecbSzdes}{\vecb_{3S}^*}
\newcommand{\vecbxdes}{\vecb_{1}^*}
\newcommand{\vecbydes}{\vecb_{2}^*}
\newcommand{\vecbzdes}{\vecb_{3}^*}
\newcommand{\vecn}{\mathbf{n}}
\newcommand{\vecna}{\vecn_a}
\newcommand{\vecnba}{\vecn_{ba}}
\newcommand{\vecg}{\mathbf{g}}
\newcommand{\vecxi}{\bm{\xi}}
\newcommand{\veceta}{\bm{\eta}}
\newcommand{\vecp}{\mathbf{p}}
\newcommand{\vecq}{\mathbf{q}}
\newcommand{\vecv}{\mathbf{v}}
\newcommand{\vecr}{\mathbf{r}}
\newcommand{\vecu}{\mathbf{u}}
\newcommand{\vecmu}{\bm{\mu}}
\newcommand{\vecomega}{\bm{\omega}}
\newcommand{\vecrho}[1]{\bm{\rho}_{#1}}
\newcommand{\hatvecrho}[1]{\hat{\bm{\rho}}_{#1}}
\newcommand{\vecrw}{\vecr^{\worldf}}
\newcommand{\vecut}{\mathbf{u}_t}
\newcommand{\vecx}{\mathbf{x}}
\newcommand{\vecxt}{\vecx_t}

%Matrix
\newcommand{\mat}[2]{\mathbf{#1}_{#2}}
\newcommand{\dotmat}[2]{\dot{\mathbf{#1}}_{#2}}
\newcommand{\matA}{\mathbf{A}}
\newcommand{\matBt}{\mathbf{B}_t}
\newcommand{\matC}{\mathbf{C}}
\newcommand{\matI}{\mathbf{I}}
\newcommand{\matK}{\mathbf{K}}
\newcommand{\matM}{\mathbf{M}}
\newcommand{\matP}{\mathbf{P}}
\newcommand{\matU}{\mathbf{U}}
\newcommand{\matR}{\bm{\mathit{R}}}
\newcommand{\matX}{\mathbf{X}}
\newcommand{\matKpS}{\mathbf{K}_{pS}}
\newcommand{\matKdS}{\mathbf{K}_{dS}}
\newcommand{\matQone}{\mathbf{Q}_{1}}
\newcommand{\matQtwo}{\mathbf{Q}_{2}}
\newcommand{\matVt}{\mathbf{V}_t}
\newcommand{\matdeltaT}{\mathbf{\Delta T}}
\newcommand{\matzero}{\mathbf{0}}
\newcommand{\matInine}{\mathbf{I}_{9\times9}}
\newcommand{\matIthree}{\mathbf{I}_{3\times3}}

%Constant
\newcommand{\inertia}{\mathbf{J}}
\newcommand{\inertiaload}{\mathbf{J}_{L}}
\newcommand{\loadmass}{m_{L}}
\newcommand{\massi}{m_{k}}
\newcommand{\massQ}{m_{Q}}
\newcommand{\half}{\frac{1}{2}}

%state
\newcommand{\angvel}{\mathbf{\Omega}}
\newcommand{\angacc}{\dot{\angvel}}

\newcommand{\robotpos}[1]{\vecx_{#1}}
\newcommand{\robotrot}[1]{\matR_{#1}}
\newcommand{\robotdotrot}[1]{\dot{\matR}_{#1}}
\newcommand{\robotvel}[1]{\dot{\vecx}_{#1}}
\newcommand{\robotacc}[1]{\ddot{\vecx}_{#1}}
\newcommand{\robotangvel}[1]{\angvel_{#1}}
\newcommand{\robotangacc}[1]{\angacc_{#1}}

\newcommand{\tension}[1]{\vecmu_{#1}}
\newcommand{\tensiondes}[1]{\vecmu_{#1,des}}
\newcommand{\loadpos}{\vecx_{L}}
\newcommand{\loadposdes}{\vecx_{L,des}}
\newcommand{\loadrot}{\matR_{L}}
\newcommand{\loadrotdes}{\matR_{L,des}}
\newcommand{\loaddotrot}{\dot{\matR}_{L}}
\newcommand{\loadvel}{\dot{\vecx}_{L}}
\newcommand{\loadveldes}{\dot{\vecx}_{L,des}}
\newcommand{\loadacc}{\ddot{\vecx}_{L}}
\newcommand{\loadaccdes}{\ddot{\vecx}_{L,des}}
\newcommand{\loadangvel}{\angvel_{L}}
\newcommand{\loadangveldes}{\angvel_{L,des}}
\newcommand{\loadangacc}{\angacc_{L}}



\newcommand{\cablevec}[1]{\vecxi_{#1}}
\newcommand{\cableveci}{\cablevec{\sy{id}}}
\newcommand{\cablevecides}{\cablevec{\sy{id},des}}
%\newcommand{\cableveci}{\vecq_{i}}
%\newcommand{\cablevec}[1]{\vecq_{#1}}
%\newcommand{\cablevecides}{\vecq_{i,des}}
\newcommand{\cablevel}[1]{\vecomega_{#1}}
\newcommand{\cableveldes}[1]{\vecomega_{#1,des}}
\newcommand{\cabledotvec}[1]{\dot{\vecxi}_{#1}}
\newcommand{\cabledotveci}{\cabledotvec{\sy{id}}}
\newcommand{\cabledotvecides}{\cabledotvec{\sy{id},des}}
\newcommand{\cableddotvec}[1]{\ddot{\vecxi}_{#1}}
\newcommand{\cableddotveci}{\cableddotvec{\sy{id}}}

\newcommand{\quat}{\vecq}
\newcommand{\quatdot}{\dot{\vecq}}
\newcommand{\rt}{\vecr_{T}}
\newcommand{\rdes}{\mathbf{r}^{*}}
\newcommand{\vecxtprev}{\mathbf{x}_{t-1}}
\newcommand{\vecntone}{\mathbf{n}_t^{1}}
\newcommand{\vecnttwo}{\mathbf{n}_t^{2}}
\newcommand{\omegai}{\bm{\omega}_{\sy{id}}}
\newcommand{\dotomegai}{\dot{\bm{\omega}}_{\sy{id}}}
\newcommand{\Omegai}{\bm{\Omega}_\sy{id}}
\newcommand{\dotOmegai}{\dot{\bm{\Omega}}_{\sy{id}}}

\newcommand{\inputforce}{\vecu}

%payload estimation
\newcommand{\point}[1]{\vecp_{#1}}

%filterstate
\newcommand{\ekfstatei}{\mat{X}{k}}
\newcommand{\ekfdotstatei}{\dotmat{X}{k}}
\newcommand{\ekfinputi}{\mat{U}{k}}
\newcommand{\acci}{\veca_{\mathit{\sy{id}}}}
\newcommand{\aptpos}[1]{\vecp_{#1}}
\newcommand{\aptvel}[1]{\dot{\vecp}_{#1}}
\newcommand{\aptacc}[1]{\ddot{\vecp}_{#1}}

%set
\newcommand{\realnum}[1]{\mathbb{R}^{#1}}
\newcommand{\SOthree}{SO(3)}

%components
\newcommand{\KpSx}{K_{pxS}}
\newcommand{\KpSy}{K_{pyS}}
\newcommand{\KpSz}{K_{pzS}}
\newcommand{\KdSx}{K_{dxS}}
\newcommand{\KdSy}{K_{dyS}}
\newcommand{\KdSz}{K_{dzS}}

\newcommand{\rotorijx}{x_{ij}}
\newcommand{\rotorijy}{y_{ij}}
\newcommand{\rotorijz}{z_{ij}}

%Operation
\newcommand{\sumn}[1]{\sum_{#1=1}^n}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\twonorm}[1]{\left\lVert#1\right\rVert_2}
\newcommand{\prths}[1]{\left(#1\right)}
\newcommand{\brcks}[1]{\left[#1\right]}
\newcommand{\robotframe}[1]{\robotf_{#1}}
\newcommand{\viocamframe}[1]{\camf_{\robotframe{#1}}}
\newcommand{\qcamframe}[1]{\camf_{#1}}
\newcommand{\axis}[2]{\mathbf{e}_{#1}^{#2}}
\newcommand{\des}{{*\mathcal{}}}

==> sections/archived.tex <==
% \begin{table}[!t]
% \caption {Notation table.\label{tab:notation}} 
% \centering
% \begin{tabularx}{0.48\textwidth}{>{\hsize=0.58\hsize}X >{\hsize=1.42\hsize}X}
%     \hline\hline
%     \hline\hline
% \end{tabularx}
% \vspace{-1em}
% \end{table}


%Moreover, a new concept of virtual physical human robot interaction needs to be introduced, especially to decrease the human physical and mental workload while increasing the common spatial awareness during the exploration. At this purpose a bidirectional communication between the two agents of various key spatial features during the collaborative exploration has been defined, increasing the intuitiveness of the human robot interaction.
%Moreover an aerial robot has been considered as human teammate since its enhanced perception capabilities, its smaller size and its ability to fly, define it as the perfect candidates to carry out tasks requiring high levels of flexibility and maneuverability, such as search and rescue operations, environmental monitoring, and infrastructure inspection.

%As envisioned in the Industry 4.0 revolution, human-robot interaction will play a more important role in future industries and daily life~\cite{Schwab_2017}. While HRI spans a broad spectrum of interaction modalities, from direct physical engagement to indirect interfaces like joysticks and tablets, the recent rise of consumer-grade augmented reality or mixed reality (MR) devices, such as the Microsoft HoloLens, Meta 2, and Apple Headset, has opened new possibilities for intuitive and immersive HRI. These devices allow the user to interact with the robot through a mixed reality interface, which can be used to visualize the robot's state, control the robot~\cite{florian2023hriAR}, supervise the robot's operation~\cite{adams2023can}, or provide feedback to the user.

%However, the majority of existing research in HRI has been focused on ground robots. Only a few approaches exist for aerial robots, mostly limited to teleoperation. Compared to ground robots, aerial robots offer unparalleled advantages in terms of 3D mobility and compactness, making them ideal candidates for tasks requiring high levels of flexibility and maneuverability, such as search and rescue operations, environmental monitoring, and infrastructure inspection.



%Our approach aims to enhance the human operator's situational awareness during exploration or inspection tasks, particularly in high-risk environments. Leveraging the Mixed Reality technology we provide to the user spatial information of the environment perceived by the robot. At each iteration 

%we have to describe here what is happening while the user is exploring and what is the innovation 

%ur approach aims to enhance the human operator's situational awareness during exploration or inspection tasks, particularly in high-risk environments meanwhile solving various challenges, mostly related to the relative localization of the user compared to the drone provided 3D map and the geometrical visualization of the drone spatial awareness in the user field of view. Moreover, a bidirectional spatial communication has been established, where also the user is sharing spatial information about his/her surroundings to the robot. 
%The framework allows the human operator to delegate exploration of potentially hazardous areas to the aerial robot while focusing on assessing less dangerous areas. %The MAV, in turn, updates the real-time mapping data back to the operator, which is visualized through the HoloLens interface. This not only relieves the need for cumbersome equipment like laptops or radio controllers but also fosters a more seamless and intuitive collaboration between the human and the MAV.

%The proposed framework has far-reaching implications, particularly for search and rescue operations where rapid decision-making can be the difference between life and death. 
%By providing a more intuitive and responsive interface, our system allows first responders to better assess risks and make more informed decisions, thereby increasing the likelihood of successful missions.

%This paper makes several key contributions to the field of HRI with aerial robots. We present a novel MR-based interface for MAVs, which enables the human operator to command, receive perception feedback from the aerial robots. elaborate on the custom algorithms developed for real-time mapping and data visualization, and validate our system through extensive real-world testing.

In the realm of human-robotic exploration, the key to enhancing task efficiency lies in maximizing flexibility, maneuverability, rapid agile movements, and user-friendly operation. To meet these requirements, the Unmanned Aerial Vehicle (UAV) emerges as the ideal candidate for the job. Our robotic system uses the capabilities of a lightweight aerial robot, the RACE quadrotor platform. It is an in-lab UAV that is fully customized in terms of hardware and software for mapping potentially hazardous areas. The RACE design is depicted in .


A nonlinear geometric controller~\cite{lee2010geometric} runs on the Jetson Xavier NX. 
As a low-level attitude controller,  is used, which runs at $800~\si{Hz}$, receiving commands from

An Intel Realsense D435i camera is used for perception and environmental awareness, which provides stereo images at $30~\si{Hz}$ and IMU data at $200~\si{Hz}$. During the flight tests in this paper, the robot operates autonomously, leveraging the onboard sensor data and following the user commands.



%Moreover, MR unique ability to overlay virtual holograms onto the real world holds the potential to provide an immediate and an intuitive understanding of the robot's environmental perception\cite{adams2023can,florian2023hriAR}.
%In order to enhance the human spatial and situational awareness 
%To attain this objective, it becomes crucial to consider various factors, including the type, representation, quality, and quantity of information exchanged between the agents. Proper calibration of these factors is essential, as it can profoundly influence the decision-making process within the collaborative team. 



%to 
%facilitate enhanced collaboration between humans and robots


%It achieves this by establishing a shared spatial perception between these two agents, bolstered by the aerial robot's autonomous capabilities. Users can navigate and instruct the robot solely through the MR visualization provided by the HMD.



%In this paper, we present an innovative framework that fosters assisted collaborative exploration between humans and aerial robots, capitalizing on the immersive capabilities offered by Human Head Mounted Devices (HMDs). Our primary aim is to facilitate seamless interaction between humans and robots by harnessing the potential of emerging technologies such as Mixed Reality (MR) and Augmented Reality (AR), which hold immense promise in the field of robotics.
%The key contributions of this paper can be summarized as follows:


\begin{equation}
 P_d(t) = 
 \begin{cases}
 p_{1d} (t - t_0) \quad if \quad t \in [t_0, t_1], \\
 p_{2d} (t - t_1) \quad if \quad t \in [t_2, t_1], \\
 \vdots \\
 p_{fd} (t - t_{f-1}) \quad if \quad t \in [t_f, t_{f-1}], \\
  \end{cases}\,.
\end{equation}
with 
\begin{equation}
 p_{id}(t) = \sum_{n=0}^{N} c_{nid}t^n, i = 1, \hdots, f
 \end{equation}

where $f$ is the number of splines, $N$ is the polynomial order and $d \in {1,2,3,4}$ corresponds to the dimension of the flat space of 
the UAV system composed by $\mathbf{y} = \left[\mathbf{x}^T \Psi \right] $, $p_{id}$ represents the $i_{th}$ polynomial making 
up the full trajectory of $P_d$, $c_{nid} \in \mathbb{R}$ is the $n^{th}$ coefficient of $p_{id}$. The trajectory planning problem can be formulated as a Quadratic Programming problem (QP) which can be defined with the following structure:
\begin{equation}
\begin{aligned}
\min_{\mathbf{c}_d} \quad & \mathbf{c}_d^T\mathbf{Q}\mathbf{c}_d\\
\textrm{s.t.} \quad & \mathbf{A}_d \mathbf{c}_d = \mathbf{b}_d\\
  & \mathbf{y}_d \leq \mathbf{G}_d \mathbf{c}_d  \leq \mathbf{z}_d \\
\end{aligned}
\end{equation}
where $\mathbf{c}_d$ is the stacked vector of all $\mathbf{c}_{id}$ vectors containing the coefficients $p_{id}$ for each polynomial $i$ composing the solution. 
The cost matrix term is defined as $\mathbf{Q} = Diag(\mathbf{Q}_1, ...., \mathbf{Q}_i, ..., \mathbf{Q}_f)$ where each $\mathbf{Q}_i \in R^{NxN}$ is the cost matrix related to each single polynomial $i$. The equality constraint for the endpoints of each spline is then composed by the term $\mathbf{b}_d$ generated by stacking together all the $\mathbf{b}_{id}$ user-defined constraints that are imposed at time $t_i$. The Matrix $\mathbf{A}_d = Diag(A_{1d}, .., \mathbf{A}_{id}, .., \mathbf{A}_{fd})$ is composed by stacking together all the $n^{th}$ derivatives for each spline $i$. 
Finally, the inequality constraints are defined between a lower bound $\mathbf{y}_d$ and upper bound $\mathbf{z}_d$ where $\mathbf{G}_d$ is composed in a similar way as $\mathbf{A}_d$.


% \begin{figure*}[!t]
%   \centering
%   \includegraphics[width=\textwidth]{figs/voxblox_result.png}
%   \caption{Experimental Results (a) Floor layout of scenario with the distributed area between drone and Human (b) Collaborative geometric representative map in the form of Voxblox  (c) Pointcloud generated by HoloLens in red and mesh representation generated by drone \label{fig:voxblox_and_mesh_representation}}
% \end{figure*}


%Deeper in details, in \textit{Task 1} the user perform a \textit{Single Waypoint Assignment}, placing the marker directly in the final location in the virtual mini-map thus commanding to the drone to initiates the navigation towards the goal, leveraging the path planning pipeline proposed in Section .. and visualized in Fig.~\ref{fig:block_diagram}.

%We organize our experiments into two distinct modalities. In \textbf{Modality 1}, participants need to pilot the drone in a cluttered scenario, as shown in Fig.~\ref{fig:intro}, while simultaneously exploring another area wearing the HoloLens headset. In \textbf{Modality 2}, participants must navigate the drone through the same post-disaster scenario, this time using conventional First-Person View (FPV) mode receiving real-time 15 Hz video streaming from the onboard camera, without direct line of sight.

%Experiments for \textbf{Modality 1} are divided into two tasks as presented in Section~\ref{sec:system_design}. Through hologram projection on screen, individuals can select one of these tasks to guide the drone in exploring the area. In Fig.~\ref{fig:intro}, \textbf{Task 1} and \textbf{Task 2} options are displayed within a blue box, allowing users to make their choice. The human operator can utilize an interactive marker, depicted as a green cube in Fig.~\ref{fig:intro}, to assign the goal location. After assigning a task to the drone for navigation, the human can then proceed to inspect another area.
%The two tasks are presented as below:
%\paragraph{Task 1: Single Waypoint Assignment.} 
%Pressing Task 1 button the human operator can locate a virtual object on the drone acquired mini-map, assigning one single final waypoint. 
%Once the waypoint has been locked into the virtual map pronouncing the voice command "publish", the drone initiates its navigation by planning a path through the unknown area, reaching the final goal while concurrently mapping the surrounding environment. 


%The human operator assigns an initial goal to a drone using an interactive hologram marker. In Task 1, the human assigns a single goal location to the drone using minimap. The drone initiates its navigation by planning a path through an unknown area, avoiding obstacles to reach the designated goal location while concurrently mapping the surrounding environment.

%\paragraph{Task 2: Trajectory Assignment.} 
%Conversely, In Task 2, the human has more authority on the drone motion, since he/she can directly draw a path $\bm{\sigma}_{W_v}$ within the mesh generated in the minimap. The path, represented as a sequence of waypoints, is interpolated with a trajectory, as visible in~\ref{fig:block_diagram}, while the drone is moving along it. 
%The JPS contributes to a safe re-planning of the resultant trajectory if a possible obstacle collision is detected in the original user provided path. 

%a human operator can draw a trajectory $\bm{\sigma}_{W_v}$ within the mesh generated in the minimap. The drone will then compute a path along this trajectory, ensuring obstacle avoidance and continued mapping of the remaining area even if the originally drawn trajectory presents collisions or is not feasible.


%In terms of the drone's autonomy performance, it demonstrated successful exploration and planning in the environment using a human-defined trajectory. In both the single waypoint and trajectory generation tasks,
%most of the time, the user drew a trajectory $\bm{\sigma}_{W_v}$ through an obstacle or quite close to the obstacle, yet each time, the drone was able to generate a trajectory with at least $0.4~\si{m}$ clearance from the obstacles. 
%In Fig.~\ref{fig:uav_path_result} (b) and (c), we can see the trajectory generated by the drone while avoiding the obstacles and also mapping the environment. 
%This create a direct contrast with the FPV approach, which requires users to manually navigate and plan paths while dodging obstacles based on video feedback, our system autonomously accomplishes these tasks. As results, the proposed MR apporach significantly alleviates the physical and mental strain on users, which is clearly noted in NASA TLX data findings.

%During the experiments, every participant demonstrates a level of comprehension regarding the drone's pose and surrounding mesh information, enabling them to draw the trajectory on the minimap effectively.


%Notably, some users, especially those without experience with MR devices, encounter difficulties with interactive markers, especially with pinching actions. This resulted in extended task completion time; however, the learning curve became better after one or two trials, and the users showed improvement in the completion time.


%Moreover, 
%our objective is to enhance and ease the human-drone interaction capabilities by creating a novel interface.
%Avoid to limit everything to the word interface. 
%From in this work to fig 1 express goal and method to reach it
%The proposed interface leverages Mixed Reality to overlay digital spatial features onto the real world to increase the user's situational awareness and understanding as visible in Fig. \ref{fig:intro}.
%Mixed and Augmented reality offers a compelling opportunity to enable multi-modal information sharing within the human-robot team based on vision \cite{HALME2018111}, gestures \cite{LIU2018355}, natural languages \cite{Pate2021}, and gaze \cite{LoiannoIcra, Pavliv2021}.

%To overcome these limitations, researchers have explored new type of interactions through the use of body-machine interfaces~\cite{nagi2014human}
%such as wearable devices that interpret the human body's motion as commands to interact with the robots~\cite{nagi2014human}. 
%Furthermore, recent studies have demonstrated the effectiveness of engaging humans with robots through haptic feedback~\cite{tsykunov2019swarmtouch}, as well as virtual and augmented reality headsets~\cite{macchini2019personalized,VaughanCRV2017,reardon2018ssrr}, opening new avenues in this field.  
%Despite recent advancements in interface design and interaction modalities, the current state of the art is still constrained to hierarchic communication models. 


%Human-Robot interfaces are crucial in determining how the human operator commands the robot and perceives the feedback. 

%During the robot operation in unknown or unstructured environments, it is vital to design easy and intuitive interfaces that can decrease inducted phenomena in the human, like "context switching" \cite{DOISY2017527} or "motion sickness" \cite{seo2017monocle}, which can compromise the task performance. This remains an open research area. One of the primary challenges involves determining the medium, type, and quantity of information that should be exchanged between humans and robots, in order to create an efficient collaboration during a shared task. 
%In addition, the interface should be intuitive enough to minimize the user's mental and physical burden relative to conventional interfaces while still facilitating seamless human-robot collaboration through shared spatial awareness.

%he representation system overcomes the known limits of a classic human-drone interaction where the drone is constrained to stay in the user's visual line of sight.


%This design can increase human-robot communication intuitiveness by using gestures and audio-based commands. In addition, it relieves the user's mental burden to manage the robot in complicated tasks or cluttered scenarios.  

%presented as a hologram in the HMD, enables users to monitor the robot status, accessing in real time the data captured by the robot sensors during the navigation. 



%\textbf{Modality 1}: Based on the MR-generated computer graphics, described in Section~\ref{sec:system_design}, coupled with the proposed autonomous robot pipeline, we provide to the user an innovative way to interact with the robot during an exploration mission. The virtual map, proposed in Fig.~\ref{fig:intro}, spatially available everywhere by the user, provides him/her insightful information about the exploration with the additional possibility to user drag or pick and place gestures to assign a new trajectory to the robot. 

%Leveraging the MR-generated computer graphics, described in Section~\ref{sec:system_design}, 
%the user can command the drone to navigate towards a remote or unknown area, placing a virtual object on the reconstructed map representation of the drone explored area. The map visualizations available to the user are proposed in Fig.~\ref{fig:intro}, and they can be consulted everywhere, even if the robotic agent is exploring another area, thanks to the ability to spatially superimpose the virtual map into the user's real surrounding environment.
%\textbf{Modality 2}: As comparison, the users have been asked to perform a similar exploration session, at this time without any MR support, but relying on standard drone operation techniques available in the industry. In this modality, as visible in Fig.~\ref{fig:HololensvsFPV}, the user is piloting the drone using velocity commands generated by a standard RC. Thanks to the onboard localization algorithm, the drone is able to hover in position if no command is provided, thus notably decreasing the piloting difficulties.To avoid the visual contact with the drone, a $15$ Hz video streaming from the front-facing drone camera is provided. 

%During the MR-assisted exploration described in \textbf{Modality 1}, the user has the possibility to choose between two type of interactions with the robotic counterparts, simply pressing one of the two blue holographic buttons, visible in Fig.~\ref{fig:intro}, and accessing to "Task 1" or either "Task 2", choosing between the \textit{Single Waypoint Assignment} or \textit{Multiple Waypoints Assignment}, as explained in Section~\ref{sec:assisted_nav}.


%Here explain the modality that are described below. needs to be inserted here in methodology while below just keeping the 




%Once called, the ``Minimap" not only shows insightful and clear spatial information of the robot explored environments but at the same time provides a communication bridge between the user and robot, enabling the possibility to assign a new trajectory to the drone, denoted as $\bm{\sigma}_W$, which is expressed in $\mathcal{F}_W$.
%Given the ability of the MR framework to recognize hand gestures, the user can simply pick and place or drag the virtual objects to easily interacts with the provided interface. 



%the MR device employs a virtual ray known as Raycast, which projects from the user's hand. This allows users to point or pinch objects through gesture-based commands. Using this pinch gesture, users can move the interactive marker to set frames and assign the trajectory $\bm{\sigma}_W$ towards a designated goal location. 


%Thanks to these advantages, the human operators can both provide inputs to the robot, flying in a different space, while leveraging the headset perception capabilities and the provide software architecture to map and to explore his surrounding space, considered safe to walk through. 

%In the ``Minimap", our MR system provides two ways to assign a navigation task to the drone. Users can assign a final goal directly, known as ``Task 1", or draw a trajectory ($\bm{\sigma}_{W_v}$), known as ``Task 2". These options are presented as virtual buttons, shown in Fig.~\ref{fig:intro}. Once a task is selected, the new goal or trajectory will be transformed into the inertial frame and sent to the drone. These tasks can be activated using the point-and-click gesture and published to the drone using the "Publish" voice command.
%hanks to the autonomous nature of our drone operators do not need to know obstacle locations in advance to assign a new trajectory, eliminating the need of continuous monitoring of the robot. 

%Once assigned, the new trajectory will be transformed using $\mathbf{T}_{W_v}^W$ into the inertial coordinate frame ($\bm{\sigma}_W$) starting from the minimap representation and broadcast to the drone ($\bm{\sigma}_{B}$) using $\bm{T}_{W}^B$. These tasks can be activated using the point-and-click gesture.  After assigning a task, the trajectory $\bm{\sigma}_W$ can be published to the drone using the "Publish" voice command. 

%If the chosen $\bm{\sigma}_W$ encounters obstacles, the drone's planning algorithms can adjust the trajectory to navigate safely around them. 

%If an intermediate waypoint in the trajectory is too close to an obstacle, the JPS node will bypass it and move on to the next waypoint. Similarly, if the goal endpoint is too close to or inside an obstacle, then the JPS node stops planning and waits at the previous safe waypoint for the user to send another goal.

%as identifies the shortest path to the destination. As explained in Algorithm~\ref{alg:path_planning}, the JPS continuously generates a set of intermediary waypoints $\mathcal{W}_{B,i}^{W}$. 
%It directs the robot to the final destination using an occupancy grid map and our polynomial trajectory generation algorithm~\cite{jeff2023planner}. If an intermediate waypoint in the trajectory is too close to an obstacle, the JPS node will bypass it and move on to the next waypoint. Similarly, if the goal endpoint is too close to an obstacle or inside an obstacle, then the JPS node stops planning and waits at the previous safe waypoint for the user to send another goal.

%\textbf{Modality 1}: Based on the MR-generated computer graphics, described in Section~\ref{sec:system_design}, coupled with the proposed autonomous robot pipeline, we provide to the user an innovative way to interact with the robot during an exploration mission. The virtual map, proposed in Fig.~\ref{fig:intro}, spatially available everywhere by the user, provides him/her insightful information about the exploration with the additional possibility to user drag or pick and place gestures to assign a new trajectory to the robot. 

%Leveraging the MR-generated computer graphics, described in Section~\ref{sec:system_design}, 
%the user can command the drone to navigate towards a remote or unknown area, placing a virtual object on the reconstructed map representation of the drone explored area. The map visualizations available to the user are proposed in Fig.~\ref{fig:intro}, and they can be consulted everywhere, even if the robotic agent is exploring another area, thanks to the ability to spatially superimpose the virtual map into the user's real surrounding environment.
%\textbf{Modality 2}: As comparison, the users have been asked to perform a similar exploration session, at this time without any MR support, but relying on standard drone operation techniques available in the industry. In this modality, as visible in Fig.~\ref{fig:HololensvsFPV}, the user is piloting the drone using velocity commands generated by a standard RC. Thanks to the onboard localization algorithm, the drone is able to hover in position if no command is provided, thus notably decreasing the piloting difficulties.To avoid the visual contact with the drone, a $15$ Hz video streaming from the front-facing drone camera is provided. 

%During the MR-assisted exploration described in \textbf{Modality 1}, the user has the possibility to choose between two type of interactions with the robotic counterparts, simply pressing one of the two blue holographic buttons, visible in Fig.~\ref{fig:intro}, and accessing to "Task 1" or either "Task 2", choosing between the \textit{Single Waypoint Assignment} or \textit{Multiple Waypoints Assignment}, as explained in Section~\ref{sec:assisted_nav}.

%After a 20 minutes training session with both the modalities, we ask each user to interact with the drone in each modality for $6$ minutes, in both cases trying to explore as much environment coverage as possible of the overall $85$ \si{m^2} provided in the cluttered environment, coming back to the take-off location at the end of each session.
%Moreover, during the task, the user was informed multiple times that the goal of the experimental session was to try to maximize the area explored in the proposed environments, independently from the proposed interface methods. 
%Finally, before starting the real session, the user has been asked to become acquainted with a 20 minutes simulated interaction with the platform, both with the Hololens and the FPV interface. 


%Enhancing Human-Drone Spatial Awareness with a Mixed Reality Interface for Drone Assisted Interactive Navigation
%Collaborative Exploration and Inspection: Enhancing Human-Robot Interaction with Mixed Reality }
% Interactive and Spatially Aware Human-Drone Navigation
% Navigate with Ease: Interactive Human-Drone Spatial Awareness
